Numerical schemes for a class of nonlocal conservation laws: a general approach

In this work we present a rather general approach to approximate the solutions of nonlocal conservation laws. In a first step, we approximate the nonlocal term with an appropriate quadrature rule applied to the spatial discretization. Then, we apply a numerical flux function on the reduced problem. We present explicit conditions which such a numerical flux function needs to fulfill. These conditions guarantee the convergence to the weak entropy solution of the considered model class. Numerical examples validate our theoretical results and demonstrate that the approach can be applied to other nonlocal problems.

==> macros.tex <==
\usepackage[english]{babel}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
%\usepackage{a4wide}
\usepackage{verbatim}
\RequirePackage{ifthen}
\RequirePackage[T1]{fontenc}
\RequirePackage{amsthm}
\RequirePackage{color}
\RequirePackage{listings} 
\RequirePackage{epstopdf}
\RequirePackage{emptypage}
\RequirePackage[nolist]{acronym}
\RequirePackage{multirow}
\RequirePackage{enumerate,enumitem}
\RequirePackage{caption}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta}
\RequirePackage{latexsym,amscd,makeidx}
\RequirePackage{exscale}
\RequirePackage{mathrsfs}
\RequirePackage{hyperref}
\RequirePackage{url}
\RequirePackage{booktabs}
\RequirePackage{esdiff}
\RequirePackage{listings}
\RequirePackage{tabularx}
\RequirePackage[sort,numbers]{natbib}
\RequirePackage{verbatim}
\RequirePackage{comment}
%\RequirePackage{cite}
\RequirePackage{cleveref}
\crefname{equation}{}{}
\Crefname{Equation}{}{}
\usepackage{pgfplots} 
\usepackage{pgfgantt}
\usepackage{pdflscape}
%\usepackage[notref,notcite]{showkeys}
\pgfplotsset{compat=newest} 
\pgfplotsset{plot coordinates/math parser=false}
\numberwithin{equation}{section}
% Switch: Hide or show comments
	\newif\ifshowcomments								
%	\showcommentstrue				% show comments
	\showcommentsfalse				% hide comments


% Definition of environments
	\definecolor{mygrey}{gray}{0.65}
	
	% Detailed comments
	\ifshowcomments
		% Display comments in a specified environment
		\newenvironment{bcomment}[1][]
	 	{~\\~\\ \begin{color}{mygrey}\begin{small}\noindent\textbf{COMMENT: #1}~\\}
	 	{\end{small}\end{color}~\\~\\}
	\else
		% Hide comments
	 	\excludecomment{bcomment}
	\fi
	% Inline-Comments
	
	\ifshowcomments
		\newcommand{\scomment}[1]{{\color{mygrey} [#1]}}  % small comments within lines
	\else
		\newcommand{\scomment}[1]{\iffalse #1 \fi}
	\fi

% Adjust sign of a number for the tikz picture of the grid 
	\newcommand\checkindex[1]{
		\pgfmathsetmacro{\var}{#1}
		\pgfmathparse{ifthenelse(\var==0, "",ifthenelse(\var>0, "+#1","#1"))} \pgfmathresult}%

%For tikz plots
\newlength\fwidth

% Create 'todo' marker (called by \todo{TEXT})
\newcommand{\margtodo}
{\marginpar{\textbf{\textcolor{red}{ToDo}}}{}}
\newcommand{\todo}[1]
{{\textbf{\textcolor{red}{-- \margtodo{}#1 --}}}{}}

\newcommand{\margidea}
{\marginpar{\textbf{\textcolor{orange}{Idea}}}{}}
\newcommand{\idea}[1]
{{\textbf{\textcolor{orange}{-- \margidea{}#1 --}}}{}}

\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\BV}{BV}

\theoremstyle{plain}						% Default
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

%%%Notation:
%Define some shortcuts
%% math calligraphy
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%% math blackboard bold
%\newcommand{\A}{\mathbb{A}}
%\newcommand{\B}{\mathbb{B}}
%\newcommand{\C}{\mathbb{C}}
%\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
%\newcommand{\I}{\mathbb{I}}
%\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
%\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\T}{\mathbb{T}}
%\newcommand{\U}{\mathbb{U}}
%\newcommand{\V}{\mathbb{V}}
%\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}

%% New commands
\newcommand{\OAP}{$(\Omega,\mathcal{A},P)$}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
\newcommand{\sign}{\operatorname{sgn}}
\newcommand{\Div}{\operatorname{div}}
\newcommand{\lano}{\mathrm{o}}
\newcommand{\lanO}{\mathrm{O}}
\newcommand{\dint}{\displaystyle\int}
\newcommand{\dsup}{\displaystyle\sup}
\newcommand{\dsum}{\displaystyle\sum}
%\newcommand{\BV}{\operatorname{BV}}
\newcommand{\TV}{\operatorname{TV}}
%System
\newcommand{\consys}{\cQ}

%Indicies
\newcommand\half{{\frac12}}
\newcommand\jmo{{j-1}}
\newcommand\jmh{{j-\half}}
\newcommand\jpmh{{j\pm\half}}
\newcommand\jph{{j+\half}}
\newcommand\jpo{{j+1}}
\newcommand{\jpk}{{j+k}}
\newcommand{\jpko}{{j+k+1}}
\newcommand{\kmo}{{k-1}}
\newcommand\npo{{n+1}}

%Step sizes
\newcommand{\Dx}{\Delta x}
\newcommand{\Dt}{\Delta t}

%Computations
\newcommand\dx{\mathit{dx}}
\newcommand\dy{\mathit{dy}}
\newcommand\dt{\mathit{dt}}
\newcommand\ds{\mathit{ds}}
\newcommand{\norm}[1]{{\left\|#1\right\|}}
\newcommand{\abs}[1]{{\left|#1\right|}}

%Spaces:
\newcommand{\LinfR}{{L^\infty(\R)}}
\newcommand{\LinfRR}{{L^\infty(\R;\R)}}
\newcommand{\LoneR}{{L^1(\R)}}
\newcommand{\LoneRR}{{L^1(\R;\R)}}
\renewcommand{\L}[1]{L^{#1}}
\newcommand{\Lloc}[1]{L^{#1}_{loc}}

%Nonlocal look ahead distance for the source term
\newcommand{\nds}{{\nu}}
%Kernel Function for source term
\newcommand{\ws}{W_{\nds}}
%Nonlocal look ahead distance for the transport term
\newcommand{\ndt}{{\eta}}
%Kernel Function for transport term
\newcommand{\wt}{\omega_{\ndt}}
\newcommand{\twt}{\tilde{\wt}}
%Upperbound for discrete convolution
\newcommand{\Ne}{N_\ndt}

%Kernel Functions transport:
\newcommand{\wtcon}{\wt^{\text{const.}}}
\newcommand{\wtlin}{\wt^{\text{lin.}}}
\newcommand{\wtconcave}{\wt^{\text{conc.}}}
%Coupling function:
\newcommand{\coupling}{g}
\newcommand{\newg}{\Gamma}
%Test functions
\newcommand{\testf}{\phi}

%Discrete rho
\newcommand{\dr}{\rho^{\Dx}}
%N_T Time iterations scheme
\newcommand{\NT}{{N_T}}

%n for different \Dx values for convergence
\newcommand{\nconv}{\mathcal{N}}

%Characteristics
\newcommand{\chr}{X}
%Characteristics of rho, t0, x0
\newcommand{\chrptxz}{{\chr_\rho[t_0,x_0]}}


%Paper Maximum Principle
\renewcommand{\P}{P}
\newcommand{\w}{w}
\newcommand{\coeff}{\mu}
\newcommand\opt{{\text{opt}}}
\newcommand\brho{{\bar\rho}}
\renewcommand{\S}{SI}

% quadrature
\newcommand{\qn}{{\nu}}
\newcommand{\nqn}{{J}}
\newcommand{\qw}{{h}}
\newcommand{\qwn}{\qw_\qn}
\newcommand{\qvar}{{y}}

%Order of reconstruction
\newcommand{\g}{o}
\newcommand{\GPopt}{O}


%For networks
\newcommand{\road}{E}
\newcommand{\roadind}{e}
\newcommand{\vertice}{Z}
\newcommand{\verticeind}{z}
\newcommand{\Ro}{\rho^{\max}_1}
\newcommand{\Rt}{\rho^{\max}_2}
\newcommand{\Rtr}{\rho^{\max}_3}
\newcommand{\Rr}{\rho^{\max}_\roadind}
\newcommand{\po}{\rho_1}
\newcommand{\pt}{\rho_2}
\newcommand{\pe}{\rho_\roadind}
\newcommand{\roadbeginohne}{a}
\newcommand{\roadbegin}{\roadbeginohne_\roadind}
\newcommand{\roadendohne}{b}
\newcommand{\roadend}{\roadendohne_\roadind}
\newcommand{\incoming}{\mathcal{I}}
\newcommand{\incomingind}{i}
\newcommand{\NI}{N_\incoming}
\newcommand{\outgoing}{\mathcal{O}}
\newcommand{\outgoingind}{o}
\newcommand{\NO}{N_\outgoing}
\newcommand{\distMatrix}{\mathbb{A}}
\newcommand{\distpar}{\alpha}
\newcommand{\priopar}{q}
\newcommand{\lipschitzcoupling}{{L_\coupling}}
\newcommand{\totaltraveltime}{TTT}
\newcommand{\outflow}{O}
\newcommand{\congestionmeasure}{CM}


\newcommand{\newgo}{\newg_{\outgoingind}}

%Multilane
\newcommand{\borho}{\boldsymbol{\rho}}
\newcommand{\bodr}{\boldsymbol{\rho}^{\Dx}}
\newcommand{\drl}{\rho^{\Dx,\ell}}
\newcommand{\caratt}[1]{{\chi_{\strut#1}}}
\newcommand{\spt}{\mathop{\rm supp}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\boV}{\boldsymbol{V^\nds}}
%Characteristics of bold rho and \ell
\newcommand{\chrl}{\chr_{\borho,\ell}}
\newcommand{\chrb}{\chr_{\borho}}

%GARZ
%Lagrangian marker
\newcommand{\lm}{\omega}
\newcommand{\vg}{u}
\newcommand{\VG}{U}

\newcommand{\jan}[1]{\textcolor{orange}{[Jan: #1]}}

\newcommand{\rv}[1]{\textcolor{blue}{#1}}
